Why Steering Works: Toward a Unified View of Language Model Parameter Dynamics

Methods for controlling large language models (LLMs), including local weight fine-tuning, LoRA-based adaptation, and activation-based interventions, are often studied in isolation, obscuring their connections and making comparison difficult. In this work, we present a unified view that frames these interventions as dynamic weight updates induced by a control signal, placing them within a single conceptual framework. Building on this view, we propose a unified preference-utility analysis that separates control effects into preference, defined as the tendency toward a target concept, and utility, defined as coherent and task-valid generation, and measures both on a shared log-odds scale using polarity-paired contrastive examples. Across methods, we observe a consistent trade-off between preference and utility: stronger control increases preference while predictably reducing utility. We further explain this behavior through an activation manifold perspective, in which control shifts representations along target-concept directions to enhance preference, while utility declines primarily when interventions push representations off the model's valid-generation manifold. Finally, we introduce a new steering approach SPLIT guided by this analysis that improves preference while better preserving utility. Code is available at https://github.com/zjunlp/EasyEdit/blob/main/examples/SPLIT.md.

==> section/formula.tex <==
% \onecolumn
% \[
% \theta_c = \frac{|f_1| + |v| + \sum_{(q, a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(a_t \mid q, a_{<t}, f_1)]}
% {|f_0| + L_c \log_2 m}.
% \]

% \begin{equation}
% \begin{aligned}
% \mathrm{Preference}(c) \triangleq 
% \mathbb{E}_{(q,a)\in\mathcal{D}_c} \left[ \frac{1}{T(a)}
%     \sum_{t=1}^{T(a)} 
%     \log P_v(a_t \mid q, a_{<t}, f_1) 
% \right]
% \end{aligned}
% \label{eq:preference_def}
% \end{equation}

% {\small
% \begin{equation}
% \mathrm{Preference}
% = 
% \frac{
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{c}}
%     \sum_{t=1}^{T(a)}
%     \big[\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{c}} T(a)
% }.
% \end{equation}
% }

% {\small
% \begin{equation}
% \mathrm{Total}
% = 
% \frac{
%     |f_1| + |v| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}\cup{D}_{pos}}
%     \sum_{t=1}^{T(a)}
%     \big[-\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     |f_0| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}\cup{D}_{pos}} T(a) \log_2 m
% }.
% \label{eq:sft_compression_score}
% \end{equation}
% }

% {\small
% \begin{equation}
% \mathrm{Margin}
% = 
% \frac{
%     |f_1| + |v| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}}
%     \sum_{t=1}^{T(a)}
%     \big[-\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     |f_0| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}} T(a) \log_2 m
% }
% -
% \frac{
%     |f_1| + |v| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{pos}}
%     \sum_{t=1}^{T(a)}
%     \big[-\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     |f_0| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{pos}} T(a) \log_2 m
% }.
% \label{eq:sft_compression_score}
% \end{equation}
% }

% {\small
% \begin{equation}
% \mathrm{\theta_{neg}}
% = 
% \frac{
%     |f_1| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}}
%     \sum_{t=1}^{T(a)}
%     \big[-\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     |f_0| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{neg}} T(a) \log_2 m
% }
% , 
% \mathrm{\theta_{pos}}
% = 
% \frac{
%     |f_1| + 
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{pos}}
%     \sum_{t=1}^{T(a)}
%     \big[-\log_2 P_v(a_t \mid q, a_{<t}, f_1)\big]
% }{
%     |f_0| +
%     \displaystyle\sum_{(q, a) \in \mathcal{D}_{pos}} T(a) \log_2 m
% }.
% \label{eq:sft_compression_score}
% \end{equation}
% }

% \begin{CJK}{UTF8}{gbsn}
% 预训练压缩率 $\theta_c$ 定义为：
% \end{CJK}
% \[
% \theta_{pre} = \frac{|f_1| + \sum_{x \in \mathcal{D}_{pre}} \sum_{t=1}^{T(x)} [-\log_2 P(x_t \mid  x_{<t}, f_1)]}
% {|f_0| + \sum_{x \in \mathcal{D}_{pre}} T(x) \log_2 m}.
% \]

% % \begin{CJK}{UTF8}{gbsn}
% % 后训练压缩率 $\theta_c$ 定义为：
% % \end{CJK}
% % \[
% % \theta_{post} = \alpha\theta_{pre} + \beta\frac{|f_1'| + |v| + \sum_{(q, a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(a_t \mid q, a_{<t}, f_1)]}
% % {\sum_{(q,a) \in \mathcal{D}_{c}} T(a) \log_2 m}
% % \]

% \begin{CJK}{UTF8}{gbsn}
% 后训练压缩率 $\theta_c$ 定义1为：
% \end{CJK}
% \[
% \theta_{post} = \frac{|f_1| + \sum_{x \in \mathcal{D}_{pre}} \sum_{t=1}^{T(x)} [-\log_2 P(x_t \mid  x_{<t}, f_1)]+|f_1'| + |v| + \sum_{(q, a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(a_t \mid q, a_{<t}, f_1’)]}
% {|f_0| + \sum_{x \in \mathcal{D}_{pre}} T(x) \log_2 m+\sum_{(q,a) \in \mathcal{D}_{c}} T(a) \log_2 m}
% \]

% \begin{CJK}{UTF8}{gbsn}
% 压缩率可以只考虑数据压缩不考虑其他协议吗？：
% \end{CJK}
% \[
% \theta_{post} = \frac{\sum_{(q, a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(a_t \mid q, a_{<t})]}
% {\sum_{(q,a) \in \mathcal{D}_{c}} T(a) \log_2 m}
% \]

% \twocolumn

% \begin{CJK}{UTF8}{gbsn}
% \section{偏好的定义}

% 在基于概率的生成式语言模型中，\textbf{偏好}（Preference）指的是模型在给定输入条件下，对某一类回答的\emph{生成倾向}。这种倾向可由模型在生成完整回答时的平均 token 对数概率进行刻画，以消除不同长度的影响。概念上，偏好反映了模型概率分布对该类型回答的整体支持程度。

% 设：
% \begin{itemize}
%     \item $\mathcal{D}_c = \{(q, a)\}$ 表示类别为 $c$ 的语料集合，其中 $c\in\mathcal{C}$ 为回答类型，例如正类$(+)$或负类$(-)$。
%     \item $T(a)$ 表示回答 $a$ 的 token 总长度。
%     \item $a_{<t}$ 表示回答中第 $t$ 个 token 之前的所有 token。
%     \item $P_v(a_t \mid q, a_{<t}, f_1)$ 表示模型（参数 $v$）在给定问题 $q$、已生成 token $a_{<t}$ 及附加条件 $f_1$ 的情况下，生成 $a_t$ 的条件概率。
% \end{itemize}

% 在此设定下，类别 $c$ 的\textbf{偏好}定义为：
% \begin{equation}
% \begin{aligned}
% &\mathrm{Preference}(c) \triangleq \\
% &\mathbb{E}_{(q,a)\in\mathcal{D}_c} \left[ \frac{1}{T(a)}
%     \sum_{t=1}^{T(a)} 
%     \log P_v(a_t \mid q, a_{<t}, f_1) 
% \right]
% \end{aligned}
% \label{eq:preference_def}
% \end{equation}

% 该定义的含义为：
% \begin{enumerate}
%     \item 内层求和：计算该类回答每个 token 的条件概率的对数，并求平均，以得到回答整体的平均 token 概率（log 空间）。
%     \item 外层期望：对类别 $c$ 的所有样本取平均，得到模型在该类回答上的平均 log-likelihood。
% \end{enumerate}

% 基于上述定义，不同类别的\emph{偏好差距}可表示为：
% \begin{equation}
% \mathrm{Gap}(c_1, c_2) = \mathrm{Preference}(c_1) - \mathrm{Preference}(c_2),
% \label{eq:preference_gap}
% \end{equation}
% 该差值刻画了模型在两类回答上的倾向性差异。
% 当 $\mathrm{Gap}(+,-) > 0$ 时，模型更偏向类别 $+$（如积极回答），反之则偏向类别 $-$（如消极回答）。
% \end{CJK}

% \begin{CJK}{UTF8}{gbsn}
% \subsection{Preference 与 $\theta$ 的关系}

% 设：
% \begin{itemize}
%     \item 类别 $c \in \{\text{pos}, \text{neg}\}$；
%     \item $L_c = \sum_{(q,a) \in \mathcal{D}_c} T(a)$ 为类别 $c$ 的总 token 数；
%     \item $m$ 为词表大小；
%     \item $|f_0|, |f_1|$ 为常数项。
% \end{itemize}

% 偏好的定义为：
% \[
% \mathrm{Preference}(c) = 
% \frac{\sum_{(q,a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} \log_2 P_v(a_t \mid q, a_{<t}, f_1)}{L_c}.
% \]

% 原始压缩评分 $\theta_c$ 定义为：
% \[
% \theta_c = \frac{|f_1| + |v| + \sum_{(q, a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(a_t \mid q, a_{<t}, f_1)]}
% {|f_0| + L_c \log_2 m}.
% \]

% 注意到：
% \[
% \sum_{(q,a) \in \mathcal{D}_c} \sum_{t=1}^{T(a)} [-\log_2 P_v(\ldots)] = -\,L_c \cdot \mathrm{Preference}(c),
% \]
% 因此有以下转换关系：

% \paragraph{用 Preference 表示 $\theta$}
% \begin{align}
% \theta_c &= \frac{|f_1| + |v| - L_c \cdot \mathrm{Preference}(c)}{|f_0| + L_c \log_2 m}, \label{eq:theta_from_pref_exact} \\
% \theta_c &\approx -\,\frac{\mathrm{Preference}(c)}{\log_2 m} \quad \text{(近似，忽略常数项)}. \label{eq:theta_from_pref_approx}
% \end{align}

% \paragraph{用 $\theta$ 表示 Preference}
% \begin{align}
% \mathrm{Preference}(c) &= \frac{|f_1| + |v| - \theta_c\left(|f_0| + L_c \log_2 m\right)}{L_c}, \label{eq:pref_from_theta_exact} \\
% \mathrm{Preference}(c) &\approx -\,\theta_c \,\log_2 m \quad \text{(近似，忽略常数项)}. \label{eq:pref_from_theta_approx}
% \end{align}

% 上述精确关系式(\ref{eq:theta_from_pref_exact})-(\ref{eq:pref_from_theta_exact})为一一对应的转换公式，而近似关系式(\ref{eq:theta_from_pref_approx})-(\ref{eq:pref_from_theta_approx})在忽略常数项、样本长度分布相对均匀的情况下成立。


% 此时，偏好差距可以使用压缩率表示为：
% \begin{equation}
% \begin{split}
% \mathrm{Gap}(c_1, c_2) &= \frac{|f_1| + |v| - \theta_{c_1}\left(|f_0| + L_{c_1} \log_2 m\right)}{L_{c_1}} \\
% &- \frac{|f_1| + |v| - \theta_{c_2}\left(|f_0| + L_{c_2} \log_2 m\right)} {L_{c_2}}, \\
% \mathrm{Gap}(c_1, c_2) 
% &\approx \left(\theta_{c_2} - \theta_{c_1}\right)\log_2 m.
% \end{split}
% \label{eq:gap_theta}
% \end{equation}

% \end{CJK}


==> section/unified_view_bak.tex <==
\section{Unified View of Dynamic Weights in Inference}
% 推理时动态权重更新
We present a unified framework for dynamic weight updates during inference, viewing parameter updates and activation steering as instances of the same formulation, and observing consistent phenomena across these approaches.

\begin{table*}[ht]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Unified Affine Form} & \textbf{Activation Impact} (\boldmath$\Delta\mathbf{h}$) & \textbf{Param. Size} \\
\midrule
Fine-tuning Weight & $(\mathbf{W} + m\,\Delta\mathbf{W})\,\mathbf{h}_i + (\mathbf{b} + m\,\Delta\mathbf{b})$ & $m\,(\Delta\mathbf{W}\,\mathbf{h}_i + \Delta\mathbf{b})$ & $d_\text{in} \times d_\text{out} + d_\text{out}$ \\
LoRA & $(\mathbf{W} + m\,\mathbf{B}\mathbf{A})\,\mathbf{h}_i + \mathbf{b}$ & $m\,(\mathbf{B}\mathbf{A}\,\mathbf{h}_i)$ & $d_\text{in} \times r + r \times d_\text{out}$ \\
Steering Vector & $\mathbf{W}\,\mathbf{h}_i + (\mathbf{b} + m\,\Delta\mathbf{b})$ & $m\,\Delta\mathbf{b}$ & $d_\text{out}$ \\
\bottomrule
\end{tabular}
\caption{
All methods in our unified framework, expressed under the affine weight-update formulation (first unification) and their corresponding activation changes $\Delta\mathbf{h}$ (second unification). 
$d_\text{in}$ and $d_\text{out}$ denote the input and output dimensions of the layer; $r$ is the LoRA rank with $r \ll \min(d_\text{in}, d_\text{out})$.
}
\label{tab:unified_methods}
\end{table*}


\subsection{Unified Dynamic Weight Formulation}
\label{unified_formulation}
We propose a unified framework that encompasses both parameter update methods and activation steering methods, by viewing them as dynamic weight update. 
In this formulation, both classes of methods can be expressed under a shared affine transformation view of intermediate representations (see Section~\ref{sec:preliminary}).

Formally, the dynamic modification of the weight matrix $\mathbf{W}$ and bias vector $\mathbf{b}$ during inference can be written as:
\begin{equation}
\mathbf{h}_{i+1} = (\mathbf{W} + m_1\,\Delta\mathbf{W})\,\mathbf{h}_i + (\mathbf{b} + m_2\,\Delta\mathbf{b}),
\label{eq:unified}
\end{equation}
where $\Delta\mathbf{W}$ and $\Delta\mathbf{b}$ are update terms, and $m_1, m_2$ are scalar scaling coefficients controlling their magnitudes. In other words, the original parameters are updated to $\mathbf{W}' = \mathbf{W} + m_1\,\Delta\mathbf{W}$ and $\mathbf{b}' = \mathbf{b} + m_2\,\Delta\mathbf{b}$ before computing the next-layer activation.

When a model weight is modified, the effect can be equivalently interpreted from the activation perspective, as a change to the activation at the corresponding position. 
In this view, diverse intervention methods are unified as adding a change term to the activation:
\begin{equation}
\Delta\mathbf{h} = m_1\,\Delta\mathbf{W}\,\mathbf{h}_i + m_2\,\Delta\mathbf{b}.
\end{equation}

Under this unified view, local weight fine-tuning, LoRA, and activation steering are all specific instances, differing only in which components are updated: local weight fine-tuning modifies both $\mathbf{W}$ and $\mathbf{b}$; LoRA modifies $\mathbf{W}$ via low-rank factors; activation steering modifies only $\mathbf{b}$. Table~\ref{tab:unified_methods} summarizes their affine forms, corresponding activation update, and parameter sizes. 

Notably, introducing explicit scaling coefficients extends traditional formulations and enables continuous control over perturbation strength, a capability that plays a central role in our subsequent analysis.


% LoRA → 改乘法项
% Steering → 改加法项
% 统一公式：
% xi+1=(W+m1ΔW)xi+(b+m2Δb)
% 两者本质都是在激活上沿某概念方向施加线性扰动，只是改变参数位置不同

\subsection{Unified Dynamics Observation}

% 定义：
% Ppreference：内部倾向强度（方向性分布）
% Putility：有效生成输出使倾向可见的概率
% Preference pref：偏好目标输出能力
% Utility Putil：完成任务的通用能力
% 输出概率正比于两者乘积：Pans 正比于 Ppref×Putil

\subsubsection{Formulation of Preference and Utility Log-Odds}
\label{sec:logodds_formulation}

\paragraph{Definitions (Preference vs.\ Utility).}
We define \textbf{Preference} as the model's inherent inclination toward a target concept, and \textbf{Utility} as its capability to successfully accomplish the task.
Preference captures the model’s latent stance, while utility captures whether it can reliably express that stance as a coherent, task-relevant answer.
For illustration, in a speech analogy, preference corresponds to the speaker's internal viewpoint, and utility corresponds to the ability to articulate this viewpoint fluently and clearly.

In what follows, we aim to disentangle these two factors by decomposing the model’s observable behavior into separate preference and utility components.

\paragraph{Notation.}
Given a query $q$, we consider a concept-\emph{positive} answer $A_p$ and a concept-\emph{negative} answer $A_n$.
We denote the model’s internal preference probabilities by $P(p_p\mid q)$ and $P(p_n\mid q)$, and the utility (task-success) probabilities by $P(u_p\mid q)$ and $P(u_n\mid q)$.

\begin{assumbox}
\paragraph{Assumption 3.1 (Preference--Utility independence).}
For a matched pair $(A_p,A_n)$, we model answer likelihood as a product of \emph{preference} and \emph{utility}:
\begin{align}
P(A_p\mid q)=P(u\mid q)\,P(p_p\mid q),\nonumber\\
P(A_n\mid q)=P(u\mid q)\,P(p_n\mid q),
\end{align}

where (i) preference is binary by construction $P(p_p\mid q)+P(p_n\mid q)=1$, and
(ii) utility is polarity-invariant for the matched pair (both are valid completions), so it is shared as $P(u\mid q)$.
\end{assumbox}

\paragraph{Two log-odds metrics.}
We use \emph{log-odds} to map a probability (or probability ratio) to an unbounded, additive scale, making changes under steering easier to compare across settings.

Concretely, under the factorization, the ratio $P(A_p\mid q)/P(A_n\mid q)$ cancels the shared utility term, yielding a \emph{preference log-odds}:
\begin{align}
\mathrm{PrefOdds}(q)
&\triangleq \log\frac{P(p_p\mid q)}{P(p_n\mid q)}
= \log\frac{P(A_p\mid q)}{P(A_n\mid q)} \nonumber\\
&= \mathcal{L}_n-\mathcal{L}_p,
\label{eq:pref-odds_main}
\end{align}
where $\mathcal{L}_p$ and $\mathcal{L}_n$ are the cross-entropy losses of producing $A_p$ and $A_n$ given $q$, using $P(A\mid q)=e^{-\mathcal{L}(A\mid q)}$.

For utility, the same assumption implies that the total probability mass assigned to the two valid polarities recovers the marginal utility probability:
$P(u\mid q)=P(A_p\mid q)+P(A_n\mid q)$, leading to
\begin{align}
\mathrm{UtilOdds}(q)
&\triangleq \log\frac{P(u\mid q)}{1-P(u\mid q)}\nonumber\\
&= \log\frac{P(A_p\mid q)+P(A_n\mid q)}{1-P(A_p\mid q)-P(A_n\mid q)} \nonumber\\
&= \log\frac{e^{-\mathcal{L}_p}+e^{-\mathcal{L}_n}}
{1-e^{-\mathcal{L}_p}-e^{-\mathcal{L}_n}}.
\label{eq:util-odds_main}
\end{align}

We provide the full derivation of the factorization implications and the loss-based computation details in Appendix~\ref{app:logodds}. 
Accordingly, we mainly use $\mathrm{PrefOdds}$ and $\mathrm{UtilOdds}$ in subsequent experiments to track how a model’s concept preference and task utility evolve as the steering strength varies.


\subsubsection{Experimental Setup and Observed Unified Dynamics}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/unified_results.png}
    \caption{
        \textbf{Unified preference and utility dynamics under steering.}
        Solid lines represent preference log-odds, and dashed lines represent utility log-odds. 
        The top panel shows steering with vector-form parameter modifications, and the bottom panel shows parametric interventions including LoRA and local weight updates. 
        Results are shown for the \texttt{Gemma-2-9B-IT} model on the \emph{AxBench} dataset, evaluated over its top 10 concept subsets. 
        The horizontal axis corresponds to the steering factor.
    }
    \label{fig:unified-steering}
\end{figure*}


\paragraph{Experimental Setup.} 
We evaluate our proposed dynamic weight update framework on two types of datasets. 
The first is a personality tendency classification task, represented by the \emph{Psychopathy} dataset. 
This dataset comprises a large number of question–answer pairs grounded in personality traits, where the model must determine whether the input aligns with the target personality tendency, with the output space restricted to \texttt{Yes} or \texttt{No}. 
The second is an open-ended text generation task, for which we selected the top 10 concept subsets from the \emph{PowerSeeking} and \emph{AxBench} datasets. 
This task requires the model to produce topic-relevant natural language responses given textual instructions, covering diverse scenarios and semantic complexities. 
Experiments are conducted using two instruction-tuned language models with different sizes and architectures: \texttt{Gemma-2-9B-IT} and \texttt{Qwen-2.5-7B-Instruct}. 
We consider three intervention forms—local weight updates, low-rank adaptation (LoRA), and vector-based updates—each trained with both language modeling and RePS objectives. 
Additionally, we evaluate a training-free vector method, \emph{DiffMean}, which constructs steering vectors directly from data without any parameter optimization. 
After constructing the intervention parameters, we compute two core metrics, including preference log-odds and utility log-odds, on the train and test sets of each dataset, as defined in equations~\eqref{eq:pref-odds} and~\eqref{eq:util-odds}. 
These metrics serve to quantify the unified dynamic behavior of different methods in terms of preference and utility, providing a principled basis for the subsequent pattern analysis.

\paragraph{Unified dynamics.} 
Experimental results show that, under the unified perspective framework, different intervention forms exhibit remarkably consistent dynamic patterns. 
As shown in Figure~\ref{fig:unified-steering}, localized weight updates, low-rank adaptation (LoRA), and vector-based interventions display highly similar overall curve shapes. 

For preference log-odds, all methods typically follow three stages when plotted against the steering factor $m$: 
when $|m|$ is small, they enter the \emph{Linear Region}, where log-odds varies approximately linearly with $m$;
this is followed by a \emph{Transitional Region}, characterized by a noticeable change in trend; finally, they reach the \emph{Convergence Region}, where the curve gradually becomes flat and stabilizes.

In contrast, utility log-odds generally reach a peak within a range of $m$ values close to zero, and in some cases peaks occur on both the positive and negative sides of $m$. 
Within this relatively small $|m|$ range, utility remains at a level close to its maximum; as $|m|$ increases beyond this range, utility declines and eventually stabilizes. 

These observations demonstrate the existence of a unified pattern in how preference and utility respond to steering across different intervention forms.



% \paragraph{Definitions.}
% We define \textbf{Preference} as the model's inherent inclination toward a specific target concept, and \textbf{Utility} as its capability to successfully accomplish the given task. 
% Preference describes the model’s latent stance or bias toward the concept of interest, while utility measures its ability to externalize that stance into a coherent, well-structured, and task-relevant answer.
% For illustration, in a speech analogy, preference corresponds to the speaker's internal viewpoint, and utility corresponds to the ability to articulate this viewpoint fluently and clearly to the audience.

% \paragraph{Notation.}
% Let \(q\) denote an input query, and let \(A_p\) and \(A_n\) represent a \emph{positive} and a \emph{negative} answer, respectively, with respect to the target concept. 
% We denote \(P(u_p \mid q)\) and \(P(u_n \mid q)\) as the probabilities that the model exhibits sufficient utility when producing \(A_p\) and \(A_n\), respectively, and \(P(p_p \mid q)\) and \(P(p_n \mid q)\) as the model’s internal preference probabilities for the positive and negative options.

% \paragraph{Assumption.}
% We assume preference and utility are independent factors that combine multiplicatively to determine the probability of an observed answer:
% \begin{equation}
% \begin{aligned}
% P(A_p \mid q) &= P(u_p \mid q) \cdot P(p_p \mid q), \\
% P(A_n \mid q) &= P(u_n \mid q) \cdot P(p_n \mid q).
% \end{aligned}
% \label{eq:answer-prob}
% \end{equation}

% Under the independence assumption \(P(u_p \mid q) = P(u_n \mid q) \triangleq P(u \mid q)\) and the normalization constraint \(P(p_p \mid q) + P(p_n \mid q) = 1\), we define two log-odds metrics.

% \paragraph{Preference log-odds.}
% \begin{equation}
% \mathrm{PrefOdds}(q) \triangleq 
% \log \frac{P(p_p \mid q)}{P(p_n \mid q)}
% = \log \frac{P(A_p \mid q)}{P(A_n \mid q)}.
% \label{eq:pref-odds}
% \end{equation}

% \paragraph{Utility log-odds.}
% The marginal utility probability (regardless of preference polarity) is
% \begin{equation}
% P(u \mid q) = P(A_p \mid q) + P(A_n \mid q).
% \end{equation}
% The utility log-odds is then defined as:
% \begin{equation}
% \label{eq:util-odds}
% \mathrm{UtilOdds}(q) \triangleq 
% \log \frac{P(u \mid q)}{1 - P(u \mid q)}.
% \end{equation}

% \paragraph{Implementation using loss.}
% In practice, \(P(A_p \mid q)\) and \(P(A_n \mid q)\) are estimated from the model’s output probabilities.
% Let \(\mathcal{L}_p\) and \(\mathcal{L}_n\) denote the log-likelihood (cross-entropy) losses of producing \(A_p\) and \(A_n\), respectively. 
% With
% \[
% P(A_p \mid q) = e^{-\mathcal{L}_p}, \quad P(A_n \mid q) = e^{-\mathcal{L}_n},
% \]
% equations~\eqref{eq:pref-odds} and \eqref{eq:util-odds} can be computed directly from the losses:
% \begin{equation}
% \mathrm{PrefOdds}(q) = \mathcal{L}_n - \mathcal{L}_p,
% \end{equation}
% \begin{equation}
% \mathrm{UtilOdds}(q) = 
% \log \frac{e^{-\mathcal{L}_p} + e^{-\mathcal{L}_n}}
% {1 - e^{-\mathcal{L}_p} - e^{-\mathcal{L}_n}}.
% \end{equation}

% % \paragraph{Limitations.}
% This formulation does not account for answer length.
% If the number of tokens differs substantially between positive and negative answers, \(P(A_p \mid q)\) and \(P(A_n \mid q)\) can be replaced with the \emph{average per-token probability} to mitigate length effects.

==> tables/app_comparision.tex <==
\begin{table*}[h!]
\small
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Method} & \textbf{Memory Optimization} & \textbf{Training Cost} & \textbf{Interpretability} & \textbf{Generalization} \\
\midrule
System-1.5~\cite{arxiv25_system_1_5} & Significant & High  & Weak & Weak \\
SoftThinking~\cite{arxiv25_soft_thinking}  & Limited    & None  & Weak & Good \\
\ours & Significant & Low   & Good & Good \\
\bottomrule
\end{tabular}
\caption{Comparison of different methods.}
\label{tab:app:comparison}
\end{table*}

